BF-STVSR: B-Splines and Fourier-Best Friends for High Fidelity Spatial-Temporal Video Super-Resolution

While prior methods in Continuous Spatial-Temporal Video Super-Resolution (C-STVSR) employ Implicit Neural Representation (INR) for continuous encoding, they often struggle to capture the complexity of video data, relying on simple coordinate concatenation and pre-trained optical flow networks for motion representation. Interestingly, we find that adding position encoding, contrary to common observations, does not improve--and even degrades--performance. This issue becomes particularly pronounced when combined with pre-trained optical flow networks, which can limit the model's flexibility. To address these issues, we propose BF-STVSR, a C-STVSR framework with two key modules tailored to better represent spatial and temporal characteristics of video: 1) B-spline Mapper for smooth temporal interpolation, and 2) Fourier Mapper for capturing dominant spatial frequencies. Our approach achieves state-of-the-art in various metrics, including PSNR and SSIM, showing enhanced spatial details and natural temporal consistency. Our code is available https://github.com/Eunjnnn/bfstvsr.

==> sec/0_abstract.tex <==
\begin{abstract}
% Recently, several studies are proposed for Continuous Spatial-Temporal Video Super Resolution (C-STVSR) that upsamples the given video in spatially and temporally at the same time with arbitrary scale. Generally, these works use Implicit Neural Representation (INR) to represent the signal continuously. However, they naively map the coordinate to an RGB value without accounting for the distinctive characteristics of the spatial and temporal axes. To address this, we propose a new pipeline for C-STVSR that considers these characteristics through the following modules: \bspline that interpolate the intermediate temporal signal smoothly leveraging the fundamental property of b-spline basis function and \fourier that interpolate the intermediate spatial signals correctly by capturing dominant frequency. Along with these modules, we can generate intermediate frames at arbitrary time with high frequency information, while maintaining the natural time consistency. Our model BF-STVSR achieves the state-of-the-art performance on C-STVSR and the source code is available on \url{https://github.com/Eunjnnn/C-STVSR-exp}. 

% Enhancing low-resolution, low-frame-rate videos to high-resolution, high-frame-rate quality videos is essential for providing plausible user experiences. This motivates the development of Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which performs spatial and temporal interpolation simultaneously at arbitrary scales. While previous studies have addressed C-STVSR by leveraging Implicit Neural Representation (INR) for continuous encoding of frame and motion features, they have naively used MLP networks without considering the unique spatial and temporal characteristics of video data. To overcome this limitation, we propose a novel C-STVSR pipeline that incorporates these characteristics via two key modules: 1) {\bspline}, which smoothly interpolates motion representations using the inherit properties of the B-spline basis function and 2) {\fourier}, which correctly interpolates the spatial representations by capturing dominant frequencies. Our method, \textbf{BF-STVSR}, achieves state-of-the-art performance in terms of PSNR and SSIM, while preserving natural temporal consistency.
% \end{abstract}

% Enhancing low-resolution, low-frame-rate videos to high-resolution, high-frame-rate quality videos is essential for providing plausible user experiences. This motivates the development of Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which performs spatial and temporal interpolation simultaneously at arbitrary scales. While previous studies have addressed C-STVSR by leveraging Implicit Neural Representation (INR) for continuous encoding of frame and motion features, they have naively concatenated target coordinates to the latent features for countinuous encoding, which is insufficient to express complex video nature. In addition, while previous work utilized an additional optical flow network to extract motion information from video, we found this can limit the model's performance on leveraging rich inherent video features. To overcome these limitations, we propose a novel C-STVSR framework that introduces two key modules, which effectively represents spatial and temporal features in video: 1) {\bspline}, which smoothly interpolates motion representations using the inherit properties of the B-spline basis function and 2) {\fourier}, which effectively interpolates the spatial representations by capturing dominant frequencies. Our method, \textbf{BF-STVSR}, achieves state-of-the-art performance in terms of PSNR and SSIM, which demonstrates .




Enhancing low-resolution, low-frame-rate videos to high-resolution, high-frame-rate quality is essential for a seamless user experience, motivating advancements in Continuous Spatial-Temporal Video Super Resolution (C-STVSR). While prior methods employ Implicit Neural Representation (INR) for continuous encoding, they often struggle to capture the complexity of video data, relying on simple coordinate concatenation and pre-trained optical flow network for motion representation.  Interestingly, we find that adding position encoding, contrary to common observations, does not improve—and even degrade—performance.
% by failing to fully capture the inherent characteristics of video data. 
This issue becomes particularly pronounced when combined with pre-trained optical flow networks, which can limit the model’s flexibility. 
% We find that these restrict the model’s flexibility and hinder its ability to fully leverage the rich information inherent in video data. 
To address these issues, we propose \textbf{BF-STVSR}, a C-STVSR framework with two key modules tailored to better represent spatial and temporal characteristics of video: 1) {\bspline} for smooth temporal interpolation, and 2) {\fourier} for capturing dominant spatial frequencies. Our approach achieves state-of-the-art PSNR and SSIM performance, showing enhanced spatial details and natural temporal consistency. Our code will be available soon. 


% While previous approaches use Implicit Neural Representation (INR) to continuously encode frame and motion features, they typically rely on simple coordinate concatenation for encoding, which falls short of capturing the complex nature of video data. Additionally, prior work incorporates optical flow networks to extract motion information, yet this can hinder the model’s ability to fully leverage the rich, inherent video features. To address these limitations, we propose a novel C-STVSR framework with two key modules tailored to video’s unique spatial and temporal characteristics: 1) {\bspline}, which enables smooth interpolation of motion by leveraging the inherent properties of the B-spline basis function, and 2) {\fourier}, which captures dominant spatial frequencies for accurate spatial interpolation. Our method, \textbf{BF-STVSR}, achieves state-of-the-art in PSNR and SSIM performance, demonstrating superior spatial detail and natural temporal consistency.





\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Enhancing low-resolution, low-frame-rate videos to high-resolution, high-frame-rate quality is crucial for delivering seamless user experiences. To address this, deep learning approaches for Video Super-Resolution (VSR) \cite{chan2021basicvsr, chan2022basicvsrpp, tian2020tdan, wang2019edvr, wang2019deformable} and Video Frame Interpolation (VFI) \cite{DAIN, choi2020channel, cheng2021multiple, gui2020featureflow, kalluri2023flavr, shi2022video, cheng2020video, qvi_nips19, xiang2020zooming} have been extensively studied. VSR typically enhances spatial resolution of target frames by leveraging information from neighboring frames, while VFI improves temporal resolution by predicting inherent motion in video data. However, many existing methods are limited by fixed scaling factors set during training, which restricts their flexibility in real-world applications. %Therefore, Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which performs spatial and temporal interpolation simultaneously at arbitrary scales, is a promising direction for overcoming these limitations.

% As the quality of video representation on display devices continues to improved, deep learning-based approaches for video super-resolution (VSR) \cite{chan2021basicvsr, chan2022basicvsrpp, tian2020tdan, wang2019edvr, wang2019deformable} and video frame interpolation (VFI) \cite{DAIN, choi2020channel, cheng2021multiple, gui2020featureflow, kalluri2023flavr, shi2022video, cheng2020video, qvi_nips19, xiang2020zooming} are also have been extensively studied. Rather than super-resolve the video frames respectively, VSR generally increases to the target frame resolution using information from reference frames. Likewise, VFI leverages temporal information, such as motion vectors, to obtain more accurate pixel values for intermediate frames. 
% However, most prior studies in these two areas are limited to operate at a fixed scale factor, pre-defined during the training. It restricts the flexible usage during the inference.

%-------------------------------------------------------------------------

% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     \includegraphics[width=1.0\linewidth]{fig/figure1_cropped.pdf}

%    \caption{BF-STVSR upsamples the video in spatial and temporal at the same time. It finds the high-frequency spatial feature by the \fourier and ensures the temporal consistency by the \bspline.}
%    \label{fig:onecol}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/figure1_re2_cropped.pdf}
    \label{fig1a}
    \caption{Illustration of BF-STVSR and results. (a) BF-STVSR captures the high-frequency spatial feature by {\fourier} and interpolates temporal information smoothly via {\bspline}. (b) Temporal visualization of the interpolated video. We visualize the changes of the interpolated frames over time $t$ for a selected x-axis (indicated by yellow vertical line in (a)). Compared to other baselines, our method excels at capturing fine details and propagating them accurately over time.} 
\end{figure}

%-------------------------------------------------------------------------

On the other hand, Implicit Neural Representation (INR) has recently garnered attention for its capability to represent signals continuously through a multi-layer perceptron (MLP), making it a promising approach for super-resolution (SR) tasks  \cite{liif, lte, btc, hu2019meta}. 
% For example, LIIF \cite{liif} takes spatial coordinates $(x,y)$ as inputs and learns a local implicit function that maps each spatial coordinate into its RGB value, enabling continuous image representation and arbitrary-scale super-resolution.
%
% INR takes coordinates as inputs and parameterize the target signals (e.g. RGB value \cite{liif}, signed distance \cite{}, occupancy \cite{}) into the continuous-domain. Inspired by this attribute, a lot of studies have been proposed for arbitrary-scale single image super-resolution (SISR), enabling upsampling to any scaling factor \cite{liif, lte, btc, hu2019meta}. 
% However, it is well-known that MLPs networks tend to capture low-frequency components more effectively than high-frequency ones, which is called spectral bias \cite{siren, tancik2020fourier}. To address this, the Local Texture Estimator (LTE) \cite{lte} proposes learning fine details by estimating dominant-frequency from low-resolution images.    
% Accordingly, several recent works extend INR concept to video \cite{chen2022vinr, chen2023motif}. It enables the simultaneous upsampling of both spatial resolution and temporal frame rate at arbitrary scales, called as Continuous Spatial-Temporal Video Super Resolution (C-STVSR). Unfortunately, there are less attention in C-STVSR compared to SISR. 
Building on these advancements, recent studies have extended INR to video data to achieve Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which enables spatial and temporal interpolation simultaneously at arbitrary scales \cite{chen2022vinr, chen2023motif}. VideoINR \cite{chen2022vinr} was the first method to map spatiotemporal coordinates ${(x,y,t)}$ to backward motion field, facilitating backward warping of spatial features to any temporal coordinate. MoTIF \cite{chen2023motif} improved on this by replacing the backward warping with forward warping, using softmax splatting \cite{niklaus2020softmax}. In addition, to facilitate the learning in an explicit way, MoTIF supply forward optical flow maps estimated between reference frames as contextual information, using RAFT \cite{teed2020raft}.

% Inspired by the arbitrary-scale SISR, VideoINR \cite{chen2022vinr} propose to map the query spatiotemporal coordinate ${(x,y,t)}$ of video to target intermediate frame RGB values. Following VideoINR, MoTIF \cite{chen2023motif} change the backward warping to forward warping and use soft-splatting \cite{niklaus2020softmax} method. Also, it utilizes pre-trained optical flow network \cite{teed2020raft} to generate temporal feature and parameterize to the intermediate motion vector. However, these works only use the fundamental concept of INR, representing discrete signals continuously without considering inherent characteristics of spatial and temporal axes, respectively. We need to center on high-frequency details from low-resolution frames in spatial axis, while ensuring smooth temporal consistency along the temporal axis. Because it requires capturing high-frequency details in spatial axis while estimating objects movement in temporal axis to generate intermediate frames, which adds significant complexity. 


% While both VideoINR and MoTIF successfully integrate INR into the C-STVSR task and demonstrate the feasibility of continuously encoding spatial features with MLPs and generating intermediate frames by warping these features based on predicted motion, they have notable limitations. They rely on MLPs to predict video motion but do not account for the inherent smoothness of video movement, which can lead to sub-optimal motion predictions. Moreover, these models struggle to capture high-frequency information in the encoded spatial features---a known issue referred to as spectral bias \cite{spectralbias, tancik2020fourier})---which leads to the generation of low-quality frames.


% While both VideoINR and MoTIF successfully integrate INR into the C-STVSR task and demonstrate the feasibility of continuously encoding spatial features with MLPs and generating intermediate frames by warping these features based on predicted motion, they have notable limitations. They directly predict video motion with simple MLPs and/or employ pre-trained external networks, which only partially account for the inherent smoothness of video movement for the motion representation modeling. As a result, this approach can yield sub-optimal motion predictions, as it fails to fully capture the complex, non-linear dynamics of natural motion. Moreover, both models struggle to capture high-frequency information in the encoded spatial features---a known issue referred to as spectral bias \cite{spectralbias, tancik2020fourier})---which leads to the generation of low-quality frames.

While VideoINR and MoTIF successfully integrate INR into the C-STVSR task, they have notable limitations. Specifically, they generate target features by encoding latent features that are simply concatenated with target coordinates, without employing advanced position encoding techniques. This is surprising, given that various position encoding methods---such as Fourier encoding \cite{mildenhall2020nerf, tancik2020fourier}---are well-established and widely used in tasks like image SR with INR due to their effectiveness, having become a conventional process \cite{lte, ltew-jaewon-lee, btc, xiao2024towards}. This straightforward approach may fall short in capturing the nuanced details of spatial and temporal features, especially for motion features, which are inherently complex and dynamic. Consequently, both models struggle to retain high-frequency information in the encoded spatial features, a well-known limitation referred to as spectral bias \cite{spectralbias, tancik2020fourier}, resulting in the generation of lower-quality frames. 

Interestingly, however, we find that simply adding position encoding does not improve---and even degrade---performance in these models, an unexpected outcome that contrasts with the general success of position encoding in enhancing INR applications \cite{ijcai2021p151, gao2023adaptive, muller2022instant, kim2022scalable}. This issue becomes particularly pronounced when combined with pre-trained optical flow networks. We conjecture that, while these networks provide useful guidance for motion representation, integrating them with position encoding can inadvertently limit the model’s flexibility to fully leverage diverse video information.

% To address these limitations, we propose a novel framework, BF-STVSR, which consist of {\bspline} (BM) and {\fourier} (FM) that handle each axis separately based on their characteristic. B-spline function is well-known basis function for constructing smooth curves or surfaces based on their basis order \cite{btc}. Following this, {\bspline} (BM) uses B-spline as basis function of temporal representation to interpolate inter-frames features and generates intermediate motion vectors. It estimates coefficient and knots of features at each reference time ($t = 0 \text{ or } 1$), and adjust each feature with dilation, which is estimated by interval of video, according to the target time $t$. Additionally, {\fourier} (FM) estimates dominant frequency and its coefficient to capture fine details in spatial features and to resolve the spectral bias, following the idea of \cite{lte}.

To address these limitations, we propose BF-STVSR, a framework consisting of two modules: {\bspline} (BM) and {\fourier} (FM), each designed to handle temporal and spatial features. First, {\bspline} (BM) utilizes B-spline function, well-known established method for constructing smooth curves or surfaces \cite{btc}. This approach well-suited for capturing the continuous nature of video motion. Next, {\fourier} (FM) represents spatial features by estimating dominant frequency information of input video frames, effectively capturing fine details. %Together, these modules serve as learned positional embeddings for each axis. 
Additionally, based on our earlier analysis, rather than directly integrating a pre-trained optical flow network into our framework, we incorporate it implicitly as a loss function during training to guide the network. This design allows the model to fully leverage the rich information inherent in video data, yielding enhanced interpolated outputs.

% In summary, our contributions can be as follows: (1) We present a new perspective that views the spatial and temporal axis separately, depending on their respective characteristics. (2) We propose novel pipeline BF-STVSR, which consist of {\bspline} for temporal axis and {\fourier} for spatial axis. (3) We achieve state-of-the-art performance on C-STVSR and demonstrate it with experiments. 

In summary, our contributions are as follows: (1) We propose BF-STVSR, a framework that independently address the spatial and temporal axes by leveraging their distinct characteristics. To achieve this, (2) we design two dedicated components, B-spline Mapper (BM) for temporal motion representation and Fourier Mapper (FM) for spatial feature representation. (3) We achieve state-of-the-art performance in C-STVSR, demonstrating the effectiveness of our approach through extensive experiments.


%-------------------------------------------------------------------------


% \begin{figure*}
%   \centering
%     \includegraphics[width=\linewidth]{fig/tmp.png}
%     \caption{Overview}
%     \label{fig:short-a}
%   \hfill
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.6\linewidth}
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=\linewidth]{fig/overview3_cropped.pdf}
%     \caption{Overview.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.15\linewidth}
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=\linewidth]{fig/bspline_cropped.pdf}
%     \caption{\bspline.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.15\linewidth}
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=\linewidth]{fig/fourier_cropped.pdf}
%     \caption{\fourier.}
%     \label{fig:short-c}
%   \end{subfigure}
%   \caption{\textbf{Architecture of our BF-STVSR.} (a) We design BF-STVSR with \fourier and \bspline. They use the same feature as inputs. (B) \fourier estimates the dominant frequency and its amplitude to help network to get high-frequency information. (c) \bspline estimates the smooth interpolated feature to get temporal consistency.}
%   \label{fig:short}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/figure_overview_cropped2.pdf} 
    % \centering
    % \begin{subfigure}{0.6\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{fig/overview_demo.png} 
    %     \caption{First Figure}
    %     \label{fig:first}
    % \end{subfigure}%
    % \hfill
    % % 두 번째 및 세 번째 그림: 각각 0.4\linewidth의 상하 배치
    % \begin{subfigure}{0.4\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{fig/fourier_demo_w.png} 
    %     \caption{Second Figure}
    %     \label{fig:second}
    %     \vspace{0.2 cm} % 그림 사이 간격
    %     \includegraphics[width=\linewidth]{fig/bspline_demo_w.png} 
    %     \caption{Third Figure}
    %     \label{fig:third}
    % \end{subfigure}
    \caption{\textbf{Schematic overview of our BF-STVSR.} (a) First, two input frames are encoded as low-resolution feature maps. Based on these features, {\fourier} predicts the dominant frequency information, while {\bspline} predicts smoothly interpolated motion, which is then processed into optical flows at an arbitrary time $t$. The frequency information is temporally propagated by being warped with the optical flows. Finally, the warped frequency information is decoded to generate high-resolution interpolated RGB frame. (b) {\fourier} estimates the dominant frequency and its amplitude to capture fine-detail information from the given frames. (c) {\bspline} estimates B-spline coefficients to model inherent motion, which smoothly interpolates motion features temporally.}
    \label{fig:main}
\end{figure*}




==> sec/2_relatedwork.tex <==
\section{Related Work}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{Arbitrary Single Image Super Resolution}

% Single Image Super Resolution (SISR) extensively studied for many years, and recently a lot of works are proposed for arbitrary scale super-resolution. LIIF \cite{liif} represents images using local implicit functions, allowing for continuous and flexible scaling to arbitrary resolutions, overcoming the limitations of traditional fixed-scale methods. Local Texture Estimator (LTE) \cite{lte} finds the coefficient of dominant frequency to capture the fine details of natural images. Similarly, B-spline Texture Coefficients Estimator (BTC) \cite{btc} used the B-spline function as basis and find the dominant coefficient especially in Screen Content Images. Following the concept of B-spline function in BTC, we propose to use this as basis function in time axis. 

Single Image Super Resolution (SISR) methods \cite{swinir, edsr, pixelshuffle, zhang2018image} have achieved impressive performance, but their reliance on fixed scales limits their applicability in real-world scenarios. To address this, several studies have proposed methods to perform super resolution at arbitrary scales \cite{liif, ultrasr, ipe, lte, btc}. LIIF \cite{liif} introduced an Implicit Neural Representation (INR) approach for super resolution, representing images continuously through local implicit functions and enabling arbitrary scale upsampling. \cite{ultrasr, ipe} further used position encoding to address the  spectral bias problem \cite{spectralbias}. Recently, LTE \cite{lte} proposed identifying dominant Fourier bases from latent features to effectively capture fine details and address spectral bias. Similarly, BTC \cite{btc} employed B-spline bases instead of Fourier bases to mitigate the Gibbs phenomenon observed in Screen Content Image Super Resolution. Inspired by these methods, we explore effective position encoding techniques for C-STVSR task, which reflect the characteristics of video data.

%-------------------------------------------------------------------------
% \subsection{Video Super Resolution}
% Video Super Resolution upsamples the given low-resolution video to high-resolution video exploiting temporal information from neighboring frames. There can be occlusion or dynamic motion in target frame, it is important to bring data from nearby frames. Video Super Resolution upsamples the given low-resolution video to high-resolution video exploiting temporal information from neighboring frames. There can be occlusion or dynamic motion in target frame, it is important to bring data from nearby frames.  

% Video Super Resolution (VSR) focuses on enhancing the resolution of low-resolution (LR) videos to high-resolution (HR) videos by leveraging temporal information from adjacent frames. To faithfully enhancing target frame with reference frame, the feature from each frame needs to be aligned to the neighboring feature. To achieve this, previous works typically leverage optical flows \cite{caballero2017real, sajjadi2018frame, chan2021basicvsr, chan2022basicvsr++, implicitresampling} or deformable convolution \cite{tian2020tdan, wang2019edvr, lin2021fdan}. Although these studies effectively address the VSR problem, they are limited by their operation at fixed scales.

% Video Super-Resolution (VSR) aims to enhance the resolution of low-resolution (LR) videos by utilizing temporal information from adjacent frames. While many methods initially relied on optical flow to align features between frames, this approach can be computationally expensive and error-prone in complex scenes \cite{caballero2017real, sajjadi2018frame}. As an alternative, deformable convolutions were introduced for more flexible and efficient alignment \cite{tian2020tdan, wang2019edvr, wang2019deformable}. Recent approaches like BasicVSR \cite{chan2021basicvsr, chan2022basicvsrpp} further optimize this process through implicit alignment and bidirectional propagation. However, many of these methods are still limited by their fixed-scale operation, leading to ongoing research into more adaptable, multi-scale solutions.

%-------------------------------------------------------------------------
% \subsection{Video Frame Interpolation}
% Video Frame Interpolation upsamples the given low frame rate video to high frame rate video exploiting temporal information from neighboring frames. There can be occlusion or dynamic motion in target frame, it is important to bring data from nearby frames. Video Frame Interpolation upsamples the given low frame rate video to high frame rate video exploiting temporal information from neighboring frames. There can be occlusion or dynamic motion in target frame, it is important to bring data from nearby frames.

% Video Frame Interpolation (VFI) aims to predict unseen frames between input frames. For effective VFI, it is essential to merge information from adjacent frames. VFI approaches can be roughly categorized into two types: implicit methods \cite{choi2020channel, gui2020featureflow, kalluri2023flavr, cheng2020video, cheng2021multiple, lee2020adacof}, which predict intermediate frames directly from adjacent frames, and explicit methods \cite{shi2022video, niklaus2018context, danier2022st, kong2022ifrnet, park2021asymmetric, reda2022film, zhang2023extracting}, which explicitly model video motion (often represented in optical flow) to aggregate adjacent frame information. 

% Video Frame Interpolation (VFI) aims to predict unseen frames between input frames to increase the frame rate of a video. Effective VFI requires merging information from adjacent frames, and approaches can be broadly categorized into two types: implicit methods \cite{choi2020channel, gui2020featureflow, kalluri2023flavr, cheng2020video, cheng2021multiple, lee2020adacof}, which directly predict intermediate frames from the input frames, and explicit methods \cite{shi2022video, niklaus2018context, niklaus2020softmax, danier2022st, kong2022ifrnet, park2021asymmetric, reda2022film, zhang2023extracting}, which model video motion, often using optical flow, to guide the interpolation. While flow-based methods commonly use backward warping, forward warping has emerged as an alternative but introduces challenges like overlapping pixel mappings, which some methods address using techniques like softmax splatting \cite{niklaus2020softmax}.

% \subsection{Video Super Resolution and Video Frame Interpolation}

% Video Super-Resolution (VSR) enhances low-resolution videos by utilizing temporal information from adjacent frames. Early methods relied on optical flow for alignment, but this approach is computationally expensive and error-prone in complex scenes \cite{caballero2017real, sajjadi2018frame}. Deformable convolutions provide more flexible alignment \cite{tian2020tdan, wang2019edvr, wang2019deformable}, and recent approaches like BasicVSR \cite{chan2021basicvsr, chan2022basicvsrpp} optimize alignment and propagation process, yet are still constrained by fixed-scale operations, spurring research into multi-scale solutions.

% Video Frame Interpolation (VFI) predicts intermediate frames to increase video frame rates. Implicit methods \cite{choi2020channel, gui2020featureflow, kalluri2023flavr, cheng2020video, cheng2021multiple, lee2020adacof} directly predict frames, while explicit methods \cite{shi2022video, niklaus2018context, niklaus2020softmax, danier2022st, kong2022ifrnet, park2021asymmetric, reda2022film, zhang2023extracting} use motion models, often with optical flow, to guide interpolation. While backward warping is common, forward warping has emerged as an alternative, though it can lead to issues like overlapping pixels, addressed by techniques like softmax splatting \cite{niklaus2020softmax}.

%-------------------------------------------------------------------------

\subsection{Spatial-Temporal Video Super Resolution}
% Video Super-Resolution (VSR) aims to enhance the resolution of low-resolution (LR) videos by utilizing temporal information from adjacent frames. While many methods initially relied on optical flow to align features between frames, this approach can be computationally expensive and error-prone in complex scenes \cite{caballero2017real, sajjadi2018frame}. As an alternative, deformable convolutions were introduced for more flexible and efficient alignment \cite{tian2020tdan, wang2019edvr, wang2019deformable}. Recent approaches like BasicVSR \cite{chan2021basicvsr, chan2022basicvsrpp} further optimize this process through implicit alignment and bidirectional propagation. However, many of these methods are still limited by their fixed-scale operation, leading to ongoing research into more adaptable, multi-scale solutions.

While conventional Video Super-Resolution (VSR) \cite{caballero2017real, sajjadi2018frame,chan2021basicvsr, chan2022basicvsrpp} and Video Frame Interpolation (VFI) \cite{choi2020channel, gui2020featureflow, kalluri2023flavr, cheng2020video, cheng2021multiple, lee2020adacof,shi2022video, niklaus2018context, niklaus2020softmax, danier2022st, kong2022ifrnet, park2021asymmetric, reda2022film, zhang2023extracting}  perform interpolation along either spatial or temporal axis, Spatial-Temporal Video Super Resolution (STVSR) conducts interpolation along both axes. Haris \textit{et al.} \cite{haris2020space} have introduced a unified framework for addressing STVSR and
Xiang \textit{et al.} \cite{xiang2020zooming} have proposed to use bidirectional deformable ConvLSTM. Although these studies demonstrate impressive performance in STVSR, they both have the limitation of only addressing STVSR at fixed scales. Recently, two works \cite{chen2022vinr, chen2023motif} have been proposed for Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which performs interpolation at arbitrary scales along both spatial and temporal axes. VideoINR \cite{chen2022vinr} is the first work on C-STVSR, which takes space-time coordinates as input and maps the corresponding RGB value in continuous manner using INR. Following this, MoTIF \cite{chen2023motif} generates temporal features using optical flow and performs forward warping to predict the interpolated high-resolution frame features. Although these studies effectively tackle the C-STVSR task, relying solely on MLPs for spatial and temporal modeling leads to difficulties in learning the characteristics of the video. In this work, we adopt Fourier basis and B-spline basis functions to model spatial and temporal features of video data to address the aforementioned difficulties.


% \subsection{Continuous Spatial-Temporal Video Super Resolution}

% There are several studies for Continuous Spatial-Temporal Video Super Resolution (C-STVSR) that can upsample in spatial and temporal domain at the same time with arbitrary scale. VideoINR \cite{chen2022vinr} is the first work to implement INR. It takes space-time coordinates as input and maps the corresponding RGB value to continuously represent the space and time axes. Following this, MoTIF \cite{chen2023motif} creates temporal features through an optical flow network RAFT \cite{teed2020raft} and perform forward warping using softmax splatting \cite{niklaus2020softmax}. However previous works rarely consider the temporal consistency and naively maps the temporal feature to motion vector. In our work, We use B-spline function as basis function to modeling the motion vector. Due to its natural characteristic of B-spline function we can get better temporal consistency .

% While VSR and VFI perform interpolation along either spatial or temporal axis, Spatial-Temporal Video Super Resolution (STVSR) conducts interpolation along both axes. \cite{haris2020space} introduced a unified framework for addressing STVSR and
% \cite{xiang2020zooming} proposed to use bidirectional deformable ConvLSTM. Although these studies demonstrate impressive performance in STVSR, they both have the limitation of only addressing STVSR at fixed scales. Recently, several works \cite{chen2022vinr, chen2023motif} present Continuous Spatial-Temporal Video Super Resolution (C-STVSR), which performs interpolation at arbitrary scales along both spatial and temporal axes. VideoINR \cite{chen2022vinr} is the first work on C-STVSR, which takes space-time coordinates as input and maps the corresponding RGB value in continuous manner using INR. Following this, MoTIF \cite{chen2023motif} generates temporal features using optical flow and performs forward warping to predict the interpolated high-resolution frame features. Although these studies effectively tackle the C-STVSR task, relying solely on MLPs for spatial and temporal modeling leads to difficulties in learning the characteristics of the video. In this work, we adopt Fourier basis and B-spline basis function to model the spatial and temporal feature to address the aforementioned difficulties.


%-------------------------------------------------------------------------
% \subsection{Cross-references}
% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}


%-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }

==> sec/3_method.tex <==
\section{Method}

\subsection{Overview} \label{3_overview}
The overall flow of our method, BF-STVSR, is illustrated in \Fref{fig:main} (a). Our framework is built upon the pipeline of MoTIF \cite{chen2023motif}.  Given two low-resolution frames $I_0^L, I_1^L \in \mathbb{R}^{3\times H \times W}$, our goal is to generate a high-resolution intermediate frame $I_t^H \in \mathbb{R}^{3\times sH \times sW}$ at any time $t \in [0, 1]$ with an arbitrary scale $s$. The encoder $E$ first takes the low-resolution frames as input and produces three latent features: $F_0^L, F_{(0,1)}^L, F_1^L \in \mathbb{R}^{C\times H \times W}$. Here, $F_0^L$ and $F_1^L$ represent the latent features of $I_0^L$ and $I_1^L$, while $F_{(0,1)}^L$ serves as a template feature for the intermediate frame, incorporating information from both input frames. Next, the latent features $F_0^L, F_1^L$ are processed by two mappers. The {\bspline} (\Sref{3_B}) predicts high-resolution optical flows to target time $t$, producing $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H \in \mathbb{R}^{2\times sH \times sW}$, while the {\fourier} (\Sref{3_F}) estimates high-resolution spatial features at target scale $s$, resulting in $F_0^H, F_1^H\in \mathbb{R}^{C\times sH \times sW}$. Finally, the high-resolution features $F_0^H, F_1^H$ are temporally propagated to the target time $t$ using forward warping based on the predicted optical flow $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H$, generating intermediate features $F_t^H$. These warped features are then concatenated with target time $t$ and $F_{(0,1)}^H$, a  nearest-neighbor upsampled version of $F_{(0,1)}^L$, and decoded to produce the high-resolution intermediate frame $I_t^H$.

% Overall pipeline of BF-STVSR is in Figure \ref{figure_1}. Given two low-resolution frames $I_0^L, I_1^L \in \mathbb{R}^{3\times H \times W}$ as input, we generate high-resolution intermediate frame $I_t^H \in \mathbb{R}^{3\times sH \times sW}$ with arbitrary scale $s$ at any time $t \in [0, 1]$. First, we take $I_0^L$ and $I_1^L$ as input of our encoder $E$. The encoder $E$ generates three latent representations $F_0^L, F_{(0,1)}^L, F_1^L \in \mathbb{R}^{C\times H \times W}$, where $F_0^L, F_1^L$ are latent features of $I_0^L, I_1^L$ and $F_{(0,1)}^L$ is template-like feature of intermediate frame that appropriately reflects both input frames. Secondly, latent features $F_0^L, F_1^L$ are used as input to each Mapper. {\bspline} (BM) generates high-resolution forward optical flow maps $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H \in \mathbb{R}^{2\times sH \times sW}$ and reliability map $Z_{0 \rightarrow t}^H, Z_{1 \rightarrow t}^H \in \mathbb{R}^{1\times sH \times sW}$ which indicates how reliable optical flow maps are. BM estimates B-spline features (i.e., coefficients, knots, and dilations) at reference time $t = 0 \text{ and } 1$ from feature maps $F_0^L, F_1^L$. To interpolate the temporal feature smoothly for temporal consistency, we choose b-spline function for time basis function (section \ref{3_B}). As well, {\fourier} (FM) maps the latent features $F_0^L, F_1^L$ to $F_0^H, F_1^H$ while maintaining high-frequency information from the features. FM predicts Fourier features (i.e., coefficients, amplitude) from latent representations $F_0^L, F_1^L$ to identify fine details (section \ref{3_F}). Next, we follow \cite{niklaus2020softmax, chen2023motif} to perform softmax splatting to make $F_t^H$ and $Z_t^H$. Lastly, $F_{(0,1)}^H$, which is bilinear upsampled of $F_{(0,1)}^L$, $F_t^H$, $Z_t^H$, and time $t$ are concatenated and decoded to high-resolution frame $I_t^H$ at time $t$.


% For motion modeling, we consider the smooth and continuous temporal consistency rather than abrupt changes. To incorporate this smoothness prior, the {\bspline} represents motion using B-spline bases, known for their effectiveness in estimating continuous signals. With this B-spline representation, {\bspline} predicts forward motion vectors $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H \in \mathbb{R}^{2\times sH \times sW}$, which capture the motion between the reference frames and the target frame at time $t$, along with reliability maps $Z_{0 \rightarrow t}^H, Z_{1 \rightarrow t}^H \in \mathbb{R}^{1\times sH \times sW}$, which indicate the reliability of the motion predictions (section \ref{3_B}). For spatial feature modeling, we use Fourier bases, which are effective in capturing high-frequency details avoiding the spectral bias in neural representation. The {\fourier} transforms $F_0^L, F_1^L$ into high-resolution latent features $F_0^H, F_1^H\in \mathbb{R}^{C\times sH \times sW}$ (section \ref{3_F}).

% and softmax splatting \cite{niklaus2020softmax}, following the approach in MoTIF \cite{chen2023motif} / and $Z_t^H$

\subsection{Temporal {\bspline}} \label{3_B}
% \paragraph{B-spline Representation for Motion Modelling}
% The temporal coherent is the most important consideration in video. Especially in case of video frame interpolation, linear motion modeling is not suit for complex and non-uniform real-world motion vector. It is crucial that objects move smoothly and continuously rather than created in a jerky manner. In order to achieve this, we use non-uniform B-spline representation as basis of temporal features, which is useful because of its smoothness and flexibility. It can defined with the generalized form:

% Effective motion modeling is critical for video enhancement tasks. If the model fails to capture the coherent video motion, the target frame cannot effectively aggregate information from neighboring frames. This challenge is amplified in the C-STVSR task, where the motions between the reference frame ($I^L_0$ or $I^L_1$) and an arbitrary intermediate frame ($I^H_t$) must be modeled. Previous works, such as VideoINR \cite{chen2022vinr} and MoTIF \cite{chen2023motif}, address this by using implicit neural representations (INR) through MLPs that take spatial-temporal coordinates as input. While INR-based motion modeling allows for the prediction of motion at arbitrary times, we found that this naive approach struggles to capture the inherent motion dynamics in the video.

Accurately predicting the motion inherent in a video is key to generating a visually plausible intermediate frame from two neighboring frames. While various techniques have been proposed in video frame interpolation (VFI) studies \cite{kalluri2023flavr, cheng2020video, niklaus2020softmax, danier2022st, kong2022ifrnet, park2021asymmetric, reda2022film, zhang2023extracting} to predict motion accurately, most of them are designed for fixed scale interpolation. Therefore, applying these methods to the C-STVSR task, which requires handling arbitrary scales, is not straightforward. To overcome this challenge, VideoINR \cite{chen2022vinr} and MoTIF \cite{chen2023motif} use implicit neural representations (INR) with MLPs that take spatiotemporal coordinates as input, enabling motion modeling at arbitrary target times $t$ and scales $s$. While INR-based motion modeling provides flexibility in motion prediction, we find that it often struggles to capture the complex, dynamic nature of motion in video.

% To address this, we assume that objects in the video move smoothly and continuously, rather than in a jerky manner. Building on this assumption, we introduce a smoothness prior for motion modeling. Inspired by BTC \cite{btc}, which interpolates low-resolution screen content images using B-spline bases, we propose modeling motion features with a B-spline representation. B-spline bases, known for their effectiveness in estimating continuous signals, are well-suited for smooth motion modeling. This can be expressed as follows:

% \begin{equation}
%     s(x, t) = c[t] \beta^n \left( \frac{x - k[t]}{d[t]} \right),
% \end{equation}
% where $t$ denotes the time index of the reference frames, and $c[t]$, $k[t]$, and $d[t]$ represent the coefficients, knots, and dilations for the B-spline representation, respectively. The definition of the $n$-th order B-spline basis and the corresponding backpropagation equations are provided in the supplementary document.


% \paragraph{{\bspline}}

% We borrow the design of LIIF \cite{liif} along with our mapper to make feature space continuously. We get encoded features $F_0^L, F_1^L$ as input and temporal implicit neural function parameterize it to create motion vectors $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H$ and reliability maps $Z_{0 \rightarrow t}^H, Z_{1 \rightarrow t}^H$ at arbitrary time $t \in [0, 1]$. Therefore, the forward motion vectors and its reliability values at coordinate $q=(x,y)$ of $F_0^H, F_1^H$ are calculated as follows:

To better represent inherent motion, we introduce {\bspline}, which leverages the B-spline representation. B-spline bases are widely known for their effectiveness in modeling continuous signals \cite{btc}, making them well-suited for capturing smooth, continuous motion in videos, where objects move smoothly and continuously, rather than in jerky manner. The detailed process of {\bspline} is described in \Fref{fig:main} (b). We modify the Space-Time Local Implicit Neural Functions (ST-INF) from MoTIF \cite{chen2023motif}, resulting in our {\bspline}. Similar to ST-INF, {\bspline} predicts high-resolution forward motion vectors $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H$ and reliability maps $Z_{0 \rightarrow t}^H, Z_{1 \rightarrow t}^H$ at arbitrary time $t \in [0, 1]$. A key difference is that our {\bspline} takes encoded features $F_0^L, F_1^L$ as input, rather than optical flows from an external network (e.g., RAFT \cite{teed2020raft}). 

In addition, rather than directly predicting motion vectors to the target time $t$, our {\bspline} $p_\psi$ models the video’s inherent motion by predicting the B-spline coefficients and knots, as described in the following equation:
% The detail process of {\bspline} is in Figure \ref{fig:main} (b). To estimate motion with the B-spline representation, we modify the Space-Time Local Implicit Neural Functions (ST-INF) in MoTIF \cite{chen2023motif}, resulting in our {\bspline}. While our {\bspline} predicts high-resolution forward motion vectors $M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H$ and reliability maps $Z_{0 \rightarrow t}^H, Z_{1 \rightarrow t}^H$ at arbitrary time $t \in [0, 1]$ similar to MoTIF \cite{chen2023motif}, it takes encoder features $F_0^L, F_1^L$ as input instead of using pre-trained optical flow network \cite{teed2020raft} to create temporal features. Additionally, the {\bspline} does not directly predict the motion vectors. Alternatively, it predicts the coefficients and knots for motion modeling with B-spline representation: 


\begin{equation}
  p_\psi(z_r, \delta_r, \hat{t}) = c_r \odot \beta^n\left(\frac{\hat{t}-k_r}{d}\right).
  \label{eq:eq3}
\end{equation}
% \begin{equation*}
%     \text{where } c_r=p_c(z_{r,n},\ \delta_r), k_r=p_k(z_{r,n}, \delta_r)\text{ and } d = p_d(g).
% \label{eq:eqb}
% \end{equation*}
% where $c_r=p_c(z_{r,n},\delta_r)$, $k_r=p_k(z_{r,n}, \delta_r)$ and $d = p_d(g)$. In detail, $z_{r,n}=F_{t_r}^L(q_r)$ is the latent feature vector at $q_r = (x_r,y_r)$, which is the point closest to the query coordinates $q = (x,y)$, and $t_r \in \{0, 1\}$ is the time index of the reference frame. $p_c$, $p_k$ and $p_d$ are the coefficient estimator ($\mathbb{R}^{C+2} \mapsto \mathbb{R}^D $), knot estimator ($\mathbb{R}^{C+2} \mapsto \mathbb{R}^D $) and the dilation estimator ($\mathbb{R}^1 \mapsto \mathbb{R}^D$). Additionally, the $\hat t=\vert t-t_r\vert$ represent the relative time distance of the predicted feature $F^H_t$ with respect to the reference frame and $\delta_r(=q-q_r)$ is the spatial relative coordinates between the query coordinates and the reference coordinates. Note that $g$ is the frame interval of the input video. After linearly projecting the predicted B-spline representation, the motion vector $Z_{t_r \rightarrow t}^H(q)$ and the reliability map $M_{t_r \rightarrow t}^H(q)$ at the query coordinates $q$ are obtained as follows:
% \begin{equation}
%   \{Z_{t_r \rightarrow t}^H(q), M_{t_r \rightarrow t}^H(q)\} = f_{\theta_b} (p_\psi(z_{r,n}, \delta_r, \hat{t}))
%   \label{eq:eq2}
% \end{equation}
% With the predicted motion vectors and reliability maps, the features $F^H_0$ and $F^H_1$ are propagated to the target time $t$ by forward warping using softmax splatting \cite{niklaus2020softmax}. By learning the underlying motion directly from the input frames, rather than mapping each arbitrary time $t$ individually, our {\bspline} achieves more robust and flexible motion modeling. Additionally, because this approach does not require optical flow inference during the inference stage, it is more efficient than previous work \cite{chen2023motif}.
Here, $c_r=p_c(z_r,\delta_r)$, $k_r=p_k(z_r, \delta_r)$, and $d = p_d(g)$. Specifically, $z_r=F_{t_r}^L(q_r)$ is the latent feature vector at the point $q_r = (x_r,y_r)$, nearest to the query coordinates $q = (x,y)$, with the reference frame time index $t_r \in \{0, 1\}$. The functions $p_c$, $p_k$, and $p_d$ are the estimators for the coefficients ($\mathbb{R}^{C+2} \mapsto \mathbb{R}^{C}$), knots ($\mathbb{R}^{C+2} \mapsto \mathbb{R}^{C}$), and dilation ($\mathbb{R}^{1} \mapsto \mathbb{R}^{C}$), respectively. $\hat{t} = |t - t_r|$ represents the relative temporal distance of the predicted feature to the reference frame, and $\delta_r(= q - q_r)$ is the spatial relative coordinate between the query and reference coordinates. Finally, $g$ is the frame interval of the input video.

After linearly projecting the predicted B-spline representation using $f_{\theta_b}$, we obtain the motion vector $Z_{t_r \rightarrow t}^H(q)$ and reliability map $M_{t_r \rightarrow t}^H(q)$ at the query coordinates $q$:
\begin{equation} \{Z_{t_r \rightarrow t}^H(q), M_{t_r \rightarrow t}^H(q)\} = f_{\theta_b} (p_\psi(z_r, \delta_r, \hat{t})). \label{eq:eq2
} \end{equation}
Using the predicted motion vectors, the spatial features $F^H_0$, $F^H_1$ and reliability maps are propagated to the target time $t$ via forward warping using softmax splatting \cite{niklaus2020softmax}. Finally, we obtain intermediate latent feature $F_t^H$ and corresponding reliability map $Z_t^H$. 
By directly learning the underlying motion from the input frames instead of individually predicting each arbitrary time $t$, our {\bspline} provides a more robust and flexible motion modeling approach. Additionally, since our method does not rely on optical flow inference during the inference stage, it is more efficient compared to previous approaches like MoTIF \cite{chen2023motif}.

% \begin{equation}
%   \{Z_{t_r \rightarrow t}^H(q), M_{t_r \rightarrow t}^H(q)\} = f_{\theta_b} (z_r, q-q_r, t-t_r)
%   \label{eq:eq1}
% \end{equation}

% To exploit positional encoding and feature embedding, we use {\bspline} and make our local temporal representation smoothly. When we add our {\bspline} $p_\psi$ in Eq. (\ref{eq:eq1}), it can be written as follows:

% \begin{equation}
%   \{Z_{t_r \rightarrow t}^H(q), M_{t_r \rightarrow t}^H(q)\} = f_{\theta_b} (p_\psi(z_r, q-q_r, t-t_r))
%   \label{eq:eq2}
% \end{equation}

% {\bspline} $p_\psi$ is consist of three estimators; (1) a coefficient estimator ($p_c : \mathbb{R}^C \mapsto \mathbb{R}^D $), (2) a knot estimator ($p_k : \mathbb{R}^C \mapsto \mathbb{R}^D $), and (3) a dilation estimator ($p_d : \mathbb{R}^1 \mapsto \mathbb{R}^D$). Accordingly, encoding function $p_\psi : (\mathbb{R}^C, \mathbb{R}^2, \mathbb{R}^1 \mapsto \mathbb{R}^D)$ is defined as :

% \begin{equation}
%   p_\psi(z_r, \delta_r, \hat{t}) = c_r \odot \beta^n\left(\frac{\hat{t}-k_r}{d}\right)
%   \label{eq:eq3}
% \end{equation}
% \begin{equation}
%     \text{where } c_r=p_c(z_r, \delta_r), k_r=p_k(z_r, \delta_r), d = p_d(g).
% \label{eq:eqb}
% \end{equation}

% $\hat{t} = concat(t, 1-t)$ is the  Therefore, target time coordinate $t$ becomes $\hat{t} = concat(t, 1-t)$ and $g$ is the constant interval of input video (e.g. 0.125) and $\delta (=q-q_r)$ is relative coordinate. $\beta^n$ is $n$-th order B-spline and we use third-order ($n = 3$). By predicting how much the feature at each reference time $t_r$ should be expressed when creating the target time coordinate $t$ feature. 



%-------------------------------------------------------------------------
\begin{table*}[]
\caption{Performance comparison on the Fixed-scale STVSR baselines on Vid4, Gopro, and Adobe240 datasets. Results are evaluated using PSNR (dB) and SSIM metrics. All frames are interpolated by a factor of $\times 4$ in the spatial axis and $\times 8$ in the temporal axis. ``\textit{Average}" refers to metrics calculated across all 8 interpolated frames, while ``\textit{Center}" refers to metrics measured using $1^{st}$, $4^{th}$ and $9^{th}$ (that is single-frame interpolation) frames of the interpolated sequence. \textbf{\textcolor{red}{Red}} and \textcolor{blue}{blue} indicate the best and the second best performance, respectively.}
\label{tab:table1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cccccc}
\hline
\begin{tabular}[c]{@{}c@{}}VFI\\ Method\end{tabular} & \begin{tabular}[c]{@{}c@{}}VSR\\ Method\end{tabular} & Vid4          & Gorpo-\textit{Center} & Gopro-\textit{Average} & Adobe-\textit{Center} & Adobe-\textit{Average} & \begin{tabular}[c]{@{}c@{}}Parameters\\ (Millions)\end{tabular} \\ \hline
SuperSloMo \cite{superslomo} & Bicubic & 22.42 / 0.5645 & 27.04 / 0.7937 & 26.06 / 0.7720 & 26.09 / 0.7435 & 25.29 / 0.7279 & 19.8 \\
SuperSloMo \cite{superslomo} & EDVR \cite{wang2019edvr} & 23.01 / 0.6136 & 28.24 / 0.8322 & 26.30 / 0.7960 & 27.25 / 0.7972 & 25.90 / 0.7682 & 19.8+20.7 \\
SuperSloMo \cite{superslomo} & BasicVSR \cite{chan2021basicvsr} & 23.17 / 0.6159 & 28.23 / 0.8308 & 26.36 / 0.7977 & 27.28 / 0.7961 & 25.94 / 0.7679 & 19.8+6.3 \\
\hline
QVI \cite{qvi_nips19} & Bicubic & 22.11 / 0.5498 & 26.50 / 0.7791 & 25.41 / 0.7554 & 25.57 / 0.7324 & 24.72 / 0.7114 & 29.2 \\
QVI \cite{qvi_nips19} & EDVR \cite{wang2019edvr} & 23.48 / 0.6547 & 28.60 / 0.8417 & 26.64 / 0.7977 & 27.45 / 0.8087 & 25.64 / 0.7590 & 29.2+20.7 \\
QVI \cite{qvi_nips19} & BasicVSR \cite{chan2021basicvsr} & 23.15 / 0.6428 & 28.55 / 0.8400 & 26.27 / 0.7955 & 26.43 / 0.7682 & 25.20 / 0.7421 & 29.2+6.3 \\
\hline
DAIN \cite{DAIN} & Bicubic & 22.57 / 0.5732 & 26.92 / 0.7911 & 26.11 / 0.7740 & 26.01 / 0.7461 & 25.40 / 0.7321 & 24.0 \\
DAIN \cite{DAIN} & EDVR \cite{wang2019edvr} & 23.48 / 0.6547 & 28.58 / 0.8417 & 26.64 / 0.7977 & 27.45 / 0.8087 & 25.64 / 0.7590 & 24.0+20.7 \\
DAIN \cite{DAIN} & BasicVSR \cite{chan2021basicvsr} & 23.43 / 0.6514 & 28.46 / 0.7966 & 26.43 / 0.7966 & 26.23 / 0.7725 & 25.23 / 0.7725 & 24.0+6.3 \\
\hline
\multicolumn{2}{c|}{ZoomingSloMo \cite{xiang2020zooming}} & 25.72 / 0.7717 & 30.69 / 0.8847 & - / - & 30.26 / 0.8821 & - / - & 11.10 \\

\multicolumn{2}{c|}{TMNet \cite{xu2021temporal}} & \textbf{\textcolor{red}{25.96 / 0.7803}} & 30.14 / 0.8696 & 28.83 / 0.8514 & 29.41 / 0.8524 & 28.30 / 0.8354 & 12.26 \\
\hline
% \multicolumn{2}{c|}{VideoINR-fixed}  & 25.78 / 0.7730 & 30.73 / 0.8850 & - / - & 30.21 / 0.8805 & - / - & 11.31 \\

\multicolumn{2}{c|}{VideoINR \cite{chen2022vinr}} & 25.61 / 0.7709 & 30.26 / 0.8792  & 29.41 / 0.8669 & 29.92 / 0.8746 & 29.27 / 0.8651 & 11.31 \\

\multicolumn{2}{c|}{MoTIF \cite{chen2023motif}}  & 25.79 / 0.7745 & \textcolor{blue}{31.04 / 0.8877} & \textcolor{blue}{30.04 / 0.8773} & \textcolor{blue}{30.63 / 0.8839} & \textcolor{blue}{29.82 / 0.8750} & 12.55 \\
\hline
\multicolumn{2}{c|}{Ours} & \textcolor{blue}{25.80 / 0.7754} & \textbf{\textcolor{red}{31.14 / 0.8893}} & \textbf{\textcolor{red}{30.20 / 0.8799}} & \textbf{\textcolor{red}{30.84 / 0.8877}} & \textbf{\textcolor{red}{30.14 / 0.8808}} & 12.68 \\

\hline
\end{tabular}%
}
\end{table*}
%-------------------------------------------------------------------------

%-------------------------------------------------------------------------
\begin{table*}[]
\caption{Performance comparison on the C-STVSR baselines for out-of-distribution scale on Gopro dataset. Results are evaluated using PSNR (dB) and SSIM metrics. All frames are interpolated by a scaling factor specified on the table and metrics calculated across all interpolated frames. \textbf{Bold} indicates the best performance. }
\label{tab:table2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Temporal Scale\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatial Scale\end{tabular} & SuperSloMo \cite{superslomo} + LIIF \cite{liif}  &   DAIN \cite{DAIN} + LIIF \cite{liif}  &   TMNet \cite{xu2021temporal}  &   VideoINR \cite{chen2022vinr}  &   MoTIF \cite{chen2023motif}  & Ours \\ 
\hline
\hline
$\times 8$ & $\times 4$ & - & - & 28.83 / 0.8514 & 29.41 / 0.8669 & 30.04 / 0.8773 & \textbf{30.20 / 0.8799 } \\
\hline
$\times 6$ & $\times 4$ & 26.70 / 0.7988 & 26.71 / 0.7998 & 30.49 / 0.8861 & 30.78 / 0.8954 & 31.56 / 0.9064 & \textbf{31.68 / 0.9082} \\
$\times 6$ & $\times 6$ & 23.47 / 0.6931 & 23.36 / 0.6902 & - & 25.56 / 0.7671 & 29.36 / 0.8505 & \textbf{29.44 / 0.8516} \\
$\times 6$ & $\times 12$ & 21.92 / 0.6495 & 22.01 / 0.6499 & - & 24.02 / 0.6900 & \textbf{25.81 / 0.7330} & 25.78 / 0.7284 \\
\hline
$\times 12$ & $\times 4$ & 25.07 / 0.7491 & 25.14 / 0.7497 & 26.38 / 0.7931 & 27.32 / 0.8141 & 27.77 / 0.8230 & \textbf{28.06 / 0.8287} \\
$\times 12$ & $\times 6$ & 22.91 / 0.6783 & 22.92 / 0.6785 & - &  24.68 / 0.7358 & 26.78 / 0.7908 & \textbf{27.06 / 0.7961} \\
$\times 12$ & $\times 12$ & 21.61 / 0.6457 & 21.78 / 0.6473 & - &  23.70 / 0.6830 & 24.72 / \textbf{0.7108} & \textbf{24.87} / 0.7096 \\
\hline
$\times 16$ & $\times 4$ & 24.42 / 0.7296 & 24.20 / 0.7244 & 24.72 / 0.7526 & 25.81 / 0.7739 & 25.98 / 0.7758 & \textbf{26.40 / 0.7844} \\
$\times 16$ & $\times 6$ & 23.28 / 0.6883 &  22.80 / 0.6722 & - & 23.86 / 0.7123 & 25.34 / 0.7527 & \textbf{25.81 / 0.7621} \\
$\times 16$ & $\times 12$ & 21.80 / 0.6481 & 22.22 / 0.6420 & - & 22.88 / 0.6659 & 23.88 / 0.6923 & \textbf{24.22 / 0.6950} \\
% \hline
% \hline
% $\times 6$ & $\times 1$ & - & - & - & 32.34 / 0.9545 & 34.77 / 0.9696 & - \\
% $\times 1$ & $\times 4$ & - & - & 33.02 / 0.9206 & 32.26 / 0.9198 & 33.84 / 0.9328 & - \\

\hline
\end{tabular}%
}
\end{table*}
%-------------------------------------------------------------------------




\subsection{Spatial {\fourier}} \label{3_F}

Even with the robust motion modeling provided by the {\bspline}, the quality of the interpolated feature $F_t^H$ depends significantly on the features propagated from $F_0^H$ and $F_1^H$. VideoINR \cite{chen2022vinr} and MoTIF \cite{chen2023motif} rely on simple MLPs to interpolate the latent features $F_0^L$ and $F_1^L$. However, implicit neural functions often struggle with capturing high-frequency details, leading to poor quality in the interpolated features, as noted in several studies \cite{spectralbias, tancik2020fourier, mildenhall2020nerf}. To address this issue, LTE \cite{lte} demonstrated that using Fourier bases for spatial feature modeling significantly improves performance in arbitrary-scale super-resolution by effectively capturing dominant frequencies. Inspired by this approach, we integrate a similar strategy into our Fourier Mapper. The detail process is illustrated in \Fref{fig:main} (c). The {\fourier} $g_\phi$ predicts the dominant frequency and its amplitude of the Fourier bases for spatial features:

% \begin{equation}
%   \{F_0^H(q), F_1^H(q)\} = g_\phi(z_{r,b}, \delta_r) = A_r \odot 
%     \begin{bmatrix}
%     \cos(\pi F_r \delta) \\
%     \sin(\pi F_r \delta)
%     \end{bmatrix}
%   \label{eq:eq_4}
% \end{equation}

\begin{equation}
    \{F_0^H(q), F_1^H(q)\} = f_{\theta_f} (g_\phi(z_r, \delta_r)), \\
\end{equation}
\begin{equation}
    \text{where } g_\phi(z_r, \delta_r) \\
     = A_r \odot 
      \begin{bmatrix}
      \cos(\pi F_r \delta_r) \\
      \sin(\pi F_r \delta_r)
      \end{bmatrix}.
  \label{eq:eq4}
\end{equation}
% \begin{equation}
%   \begin{aligned}
%     \{F_0^H(q), F_1^H(q)\} &= g_\phi(z_{r,b}, \delta_r) \\
%     &= A_r \odot 
%       \begin{bmatrix}
%       \cos(\pi F_r \delta) \\
%       \sin(\pi F_r \delta)
%       \end{bmatrix}
%   \end{aligned}
%   \label{eq:eq4}
% \end{equation}
% \begin{equation}
%     \text{where } A_r = g_a(z_r), \quad F_r = g_f(z_r).
%     \label{eq:eq9}
% \end{equation}
Here, $A_r = g_a(z_r)$ and $F_r = g_f(z_r)$. Same as {\bspline}, $z_r = F_{t_r}^L(q_r)$ is the nearest latent feature vector from the query coordinates $q = (x, y)$ and $\delta_r(=q-q_r)$ is the relative coordinates in spatial domain. The $g_a$ and $g_f$ are the amplitude estimator ($\mathbb{R}^{C} \mapsto \mathbb{R}^{2C}$) and the frequency estimator ($\mathbb{R}^{C} \mapsto \mathbb{R}^{2C}$), respectively. By predicting dominant frequencies of query points in latent space, {\fourier} improves the frequency details of the interpolated features $\hat{F}_0^H$ and $\hat{F}_1^H$. After all, by linearly projecting it to $F_0^H$ and $F_1^H$ using $f_{\theta_f}$, which in turn enhances the quality of $F_t^H$. Note that, unlike LTE, which interpolates the estimated amplitude and frequency from low-resolution domain, our method estimates each coefficients in high-resolution domain and does not estimate the phase. 
% Similar to {\bspline}, we use spatial implicit neural function along with our {\fourier}. It maps the encoded low-resolution feature $F_0^L, F_1^L$ to high-resolution feature $F_0^H, F_1^H$ and embed it into Fourier space to better understand high-frequency information. When we put our {\fourier} $w_\phi$ with implicit neural function, the high-resolution features at a coordinate $q=(x,y)$ are defined as follows:
% \begin{equation}
%   \{F_0^H(q), F_1^H(q)\} = f_{\theta_f} (g_\phi(z_r, q-q_r))
%   \label{eq:eq4}
% \end{equation}
% {\fourier} $g_\phi$ is consist of two parts; (1) an amplitude parts ($g_a : \mathbb{R}^D \mapsto \mathbb{R}^C $) and (2) a frequency parts ($g_f : \mathbb{R}^D \mapsto \mathbb{R}^C $). The encoding function $g_\phi$ estimates dominant frequencies and relative Fourier coefficients to represent local representation. Given relative coordinate $\delta (=q-q_r)$ and encoded feature, {\fourier} is defined as:
% \begin{equation}
%     g_{\phi}(z_r, \delta) = A_r \odot 
%     \begin{bmatrix}
%     \cos(\pi F_r \delta) \\
%     \sin(\pi F_r \delta)
%     \end{bmatrix},
%     \label{eq:eq8}
% \end{equation}
% \begin{equation}
%     \text{where } A_r = g_a(z_r), \quad F_r = g_f(z_r).
%     \label{eq:eq9}
% \end{equation}

%  $A_r$ is amplitude vector at coordinate $z_r$ and $F_r$ is frequency matrix at coordinate $z_r$. This two estimators consist of convolution network and we understand it to get the dominant information of spatial space. Once we predict the dominant frequency, we can find features with better high-frequency information.



\subsection{Training Objective} \label{3_Loss}

We follow \cite{chen2023motif} to train our model end-to-end : 
\begin{equation}
    \mathcal{L} = \mathcal{L}_{\text{char}}(\hat{I}_t^H, I_t^H) + \beta \sum_{i=0}^{1} \mathcal{L}_{\text{char}}(\hat{M}_{i \rightarrow t}^H, M_{i \rightarrow t}^H),
    \label{eq:eq_loss}
\end{equation}
where $\mathcal{L}_{\text{char}}$ is Charbonnier loss and $\beta$ is a hyper-parameter which set as 0.01. The $\hat{I}_t^H$ is the ground-truth high-resolution frame at time $t$ and $\hat{M}_{i \rightarrow t}^H$ is the predicted optical flow from the RAFT \cite{teed2020raft}. Note that we use RAFT only to guide our {\bspline} during training.



==> sec/4_experiments.tex <==

%-------------------------------------------------------------------------
% \begin{figure*}[!t]
%     \centerline{\includegraphics[width=\textwidth]{fig/figure3_x8_overlap_cropped.pdf}}
%     \centerline{\includegraphics[width=\textwidth]{fig/figure3_x6_overlap_cropped.pdf}}
%     \caption{Qualitative comparison between previous C-STVSR methods on arbitrary scale temporal interpolation. The figure above shows the interpolated results on out-of-distribution time scale ($\times 6$), which is not seen during training. ``Overlap" refers to the averaged image of two input frames. The $x$-axis refers to the methods while the $y$-axis represents interpolated time.}
    
%     \label{figure_1} 
% \end{figure*}

\begin{figure*}[!t]
    \centerline{\includegraphics[width=\linewidth]{fig/figure3_3ex_cap_cropped.pdf}}
    \caption{Qualitative comparison on arbitrary scale temporal interpolation. ``Overlap'' refers to the averaged image of two input frames ($t=0,1$), and the following images are interpolation results at $t=(0,1)$. (a) shows the interpolated results on in-distribution time scale ($\times 8$), used during training. (b) shows the out-of-distribution time scale ($\times 6$), not seen during training. }
    
    \label{figure3} 
\end{figure*}


%-------------------------------------------------------------------------

% \begin{table*}[]
% \centering
% \caption{ Comparison of $\Delta$MoTIF and $\Delta$Ours at different space and time scales. $\Delta$ indicates the degradation PSNR(dB) / SSIM value as the temporal scale increases, while keeping the spatial scale constant. $(\cdot, \cdot)$ represents the change from the left scale to the right scale. Smaller values mean less degradation.}
% \label{tab:table-delta}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \hline
% Space scale  & \multicolumn{4}{c|}{$\times$4} & \multicolumn{3}{c|}{$\times$6} & \multicolumn{3}{c}{$\times$12}                \\
% \hline
% Time Scale & $\times$8 (in) & $($\times$6, $\times$12)$ & $($\times$12, $\times$16)$ & $($\times$16, $\times$32)$ & $($\times$6, $\times$12)$ & $($\times$12, $\times$16)$ & $($\times$16, $\times$32)$ & $($\times$6, $\times$12)$ & $($\times$12, $\times$16)$ & $($\times$16, $\times$32)$ \\
% \hline
% \hline
% $\Delta\text{MoTIF}$ & 30.04 / 0.8773 & 3.79 / 0.083 & 1.79 / 0.047 & 3.63 / 0.099 & 2.58 / 0.060 & 1.44 / 0.038 & 3.10 / 0.084 & 1.09 / 0.022 & 0.84 / 0.019 & 2.31 / 0.051       \\
% \hline
% $\Delta\text{Ours}$ & 30.20 / 0.8799 & 3.62 / 0.080  & 1.66 / 0.044 & 3.61 / 0.098 & 2.38 / 0.056 & 1.25 / 0.034 & 2.91 / 0.079 & 0.91 / 0.019 & 0.65 / 0.015 & 1.77 / 0.040      \\ 
% \hline
% \end{tabular}%
% }
% \end{table*}

%-------------------------------------------------------------------------

% \begin{table*}[]
% \centering
% \caption{Comparison of $\Delta$MoTIF and $\Delta$Ours at different space and time scales. $\Delta$ indicates the degradation PSNR(dB) / SSIM value as the temporal scale increases, while keeping the spatial scale constant. $(\cdot, \cdot)$ represents the change from the left scale to the right scale. Smaller values mean less degradation.}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \hline
% \hline
% Spatial scale  & \multicolumn{4}{c|}{$\times$4}                   & \multicolumn{3}{c|}{$\times$6}  & \multicolumn{3}{c}{$\times$12} \\
% \hline
% Temporal scale & \multicolumn{1}{c|}{$\times$8}  & \multicolumn{1}{c|}{$\times$6}  & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c|}{$\Delta(\times\text{16})$} & \multicolumn{1}{c|}{$\times$6}    & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c|}{$\Delta(\times\text{16})$} & \multicolumn{1}{c|}{$\times$6}    & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c}{$\Delta(\times\text{16})$} \\
% \hline
% \hline
% MoTIF\cite{chen2023motif}          & \multicolumn{1}{c|}{30.04 / 0.8773} & \multicolumn{1}{c|}{31.56 / 0.9064} & \multicolumn{1}{c|}{-3.79 / -0.083}  & \multicolumn{1}{c|}{-5.58 / -0.1306}  & \multicolumn{1}{c|}{29.36 / 0.8505} & \multicolumn{1}{c|}{-2.58 / -0.059}  & \multicolumn{1}{c|}{-4.02 / -0.097}  & \multicolumn{1}{c|}{25.81 / 0.7330} & \multicolumn{1}{c|}{-1.09 / -0.022}  & \multicolumn{1}{c}{-1.93 / -0.040}  \\
% \hline
% Ours           & \multicolumn{1}{c|}{30.20 / 0.8799} & \multicolumn{1}{c|}{31.68 / 0.9082} & \multicolumn{1}{c|}{-3.62 / -0.079}  & \multicolumn{1}{c|}{-5.28 / -0.123}  & \multicolumn{1}{c|}{29.44 / 0.8516} & \multicolumn{1}{c|}{-2.38 / -0.055}  & \multicolumn{1}{c|}{-3.63 / -0.089}  & \multicolumn{1}{c|}{25.78 / 0.7284} & \multicolumn{1}{c|}{-0.91 / -0.018}  & \multicolumn{1}{c}{-1.56 / -0.033}    \\
% \hline
% \end{tabular}%
% }
% \end{table*}

%-------------------------------------------------------------------------

\begin{table*}[]
\centering
\caption{Comparison of the degradation gap as the scale increases with various arbitrary scales in both axes. We measure the performance drop when the temporal scale is increased compared to the temporal scale $\times\text{6}$ at the corresponding spatial scale. Results are evaluated using PSNR (dB) and SSIM metrics. The larger (-) value means greater performance degradation.}
\label{tab:table-delta}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c||ccc||ccc||ccc}
\hline
Spatial scale  & \multicolumn{3}{c|}{$\times$4}                   & \multicolumn{3}{c|}{$\times$6}  & \multicolumn{3}{c}{$\times$12} \\
\hline
Temporal scale  & \multicolumn{1}{c|}{$\times$6}  & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c|}{$\Delta(\times\text{16})$} & \multicolumn{1}{c|}{$\times$6}    & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c|}{$\Delta(\times\text{16})$} & \multicolumn{1}{c|}{$\times$6}    & \multicolumn{1}{c|}{$\Delta(\times\text{12})$} & \multicolumn{1}{c}{$\Delta(\times\text{16})$} \\
\hline
MoTIF \cite{chen2023motif}   & \multicolumn{1}{c|}{31.56 / 0.906} & \multicolumn{1}{c|}{-3.79 / -0.083}  & \multicolumn{1}{c|}{-5.58 / -0.130}  & \multicolumn{1}{c|}{29.36 / 0.850} & \multicolumn{1}{c|}{-2.58 / -0.059}  & \multicolumn{1}{c|}{-4.02 / -0.097}  & \multicolumn{1}{c|}{25.81 / 0.733} & \multicolumn{1}{c|}{-1.09 / -0.022}  & \multicolumn{1}{c}{-1.93 / -0.040}  \\
\hline
Ours          & \multicolumn{1}{c|}{31.68 / 0.908} & \multicolumn{1}{c|}{-3.62 / -0.079}  & \multicolumn{1}{c|}{-5.28 / -0.123}  & \multicolumn{1}{c|}{29.44 / 0.851} & \multicolumn{1}{c|}{-2.38 / -0.055}  & \multicolumn{1}{c|}{-3.63 / -0.089}  & \multicolumn{1}{c|}{25.78 / 0.728} & \multicolumn{1}{c|}{-0.91 / -0.018}  & \multicolumn{1}{c}{-1.56 / -0.033}    \\
\hline
\end{tabular}%
}
\end{table*}

%-------------------------------------------------------------------------

\section{Experiments}
\subsection{Experiments Setup}


\paragraph{Implementation and Training Details}

To our knowledge, VideoINR \cite{chen2022vinr} and MoTIF \cite{chen2023motif} are the only models addressing C-STVSR. Since both models employ identical training and testing scheme, we follow the same approach unless otherwise noted. We adopt the same two-stage training strategy: for the first 450,000 iterations, the spatial scaling factor is fixed as 4, while for the remaining 150,000 iterations, it is uniformly sampled from $[1,4]$. We use the Adam optimizer with parameters $\beta_1 = 0.9$ and $\beta_2 = 0.999$, and apply cosine annealing to decay the learning rate from $10^{-4}$ to $10^{-7}$ for every 150,000 iterations. ZoomingSlowMo \cite{xiang2020zooming} is used as the encoder, with a batch size of 32, and random rotation and horizontal-flipping for data augmentation. To ensure training stability, we substitute the predicted forward motion with the ground-truth forward motion with a certain probability, starting from 1.0 and gradually reducing to 0 over the first 150,000 iterations. For {\bspline}, we use the three-layer SIRENs as the coefficient and knot estimators, and a single fully connected layer as the dilation estimator. In {\fourier}, we use three-layer SIRENs as the amplitude and frequency estimators, followed by a 3$\times$3 convolution for spatial encoding. Both {\bspline} and {\fourier} have hidden dimensions of 64, with SIREN layer dimensions set to 64, 64, and 256. %Additional network details are in the supplementary document.

\paragraph{Datasets}
We use the Adobe240 dataset \cite{su2017deep} for training, which consists of 133 videos in 720P taken by hand-held cameras. We split these videos into 100 for training, 16 for validation, and 17 for test. During training, nine sequential frames are selected from the video and the $1^{st}$ and $9^{th}$ frames are used as input reference frames. Three frames are then randomly sampled between them and used as the target ground-truth frames. 
For evaluation, we use Vid4\cite{vid4}, Adobe240 \cite{adobe240}, and Gopro \cite{Nah_2017_CVPR} datasets. Unless otherwise specified, the default spatial scale is 4, while the temporal scaling factor varies across datasets. For Vid4, temporal scale is set to $\times$2 corresponding to single frame interpolation. For Adobe240-\textit{Average} and Gopro-\textit{Average}, the temporal scale is set as $\times$8, representing multi-frame interpolation. Additionally, for Adobe240-\textit{center} and Gopro-\textit{Center}, evaluation is performed only on the center frames (\textit{i.e.}, the  $1^{st}$, $4^{th}$, $9^{th}$ frames).

\paragraph{Baseline methods}
We categorize baeline models into two types---continuous and fixed-scale---and conduct comparisons within each category. Here, Fixed-scale Space-Time Video Super-Resolution (Fixed-STVSR) are limited to super-resolving at fixed scaling factors in both axes that are learned during the training. First, we select two-stage Fixed-STVSR methods that combine fixed video super-resolution models (\textit{e.g.}, Bicubic Interpolation, EDVR \cite{wang2019edvr}, BasicVSR \cite{chan2021basicvsr}) with video frame interpolation models (\textit{e.g.}, SuperSloMo \cite{superslomo}, QVI \cite{qvi_nips19}, DAIN \cite{DAIN}). Second, we select one-stage Fixed-STVSR method, specifically ZoomingSlowMo \cite{xiang2020zooming}. For continuous methods, we select two-stage C-STVSR methods that combine continuous image super-resolution models (\textit{e.g.}, LIIF \cite{liif}) with video frame interpolation models (\textit{e.g.}, SuperSloMo \cite{superslomo}, DAIN \cite{DAIN}). Lastly, we select one-stage C-STVSR methods, including TMNet \cite{xu2021temporal}, VideoINR \cite{chen2022vinr}, and MoTIF\cite{chen2023motif}. Note that TMNet is limited to $\times$4 spatial super-resolution. 
 

%-------------------------------------------------------------------------

\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{fig/figure_tx12_yellow_cropped.pdf}

   \caption{Qualitative comparison on a large out-of-distribution scale with a spatial scale of $\times\text{4}$ and a temporal scale of $\times\text{12}$. Three interpolation results at $t= \text{0.25, 0.5, 0.75}$ are shown with residual intensity maps compared to the ground truth frame.}
   \label{fig:fig4}
\end{figure}

%-------------------------------------------------------------------------


\paragraph{Metrics}
We use Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity Index (SSIM) on the Y channel to evaluate the model performance.


\subsection{Quantitative results}

We compare our model with Fixed-STVSR methods in \Tref{tab:table1}. For single-frame interpolation tasks in STVSR, including Vid4, GoPro-\textit{Center}, and Adobe-\textit{Center}, our model achieves the best performance on all datasets except Vid4. On Vid4, TMNet outperforms other models, likely due to its training on the Vimeo90K dataset \cite{xue2019video}, which has characteristics similar to Vid4. For multi-frame interpolation tasks in STVSR, represented by GoPro-\textit{Average} and Adobe-\textit{Average}, our model surpasses the performance of the state-of-the-art MoTIF model, which uses a pre-trained optical flow network \cite{teed2020raft} to generate temporal features during training. This improvement suggests that the {\bspline} and {\fourier} components in our model provide more robust temporal and spatial feature representations.



%-------------------------------------------------------------------------
% \begin{table}[]
% \centering
% \caption{}
% \label{tab:optical_abl}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|c|c||cc}
% \hline
% B & F & O{$\cdot$}F & \multicolumn{1}{c}{Gopro}  & \multicolumn{1}{c}{Adobe}  \\ \hline \hline
% {\xmark}        & {\xmark}       & {\cmark}            & \multicolumn{1}{c}{30.04 / 0.8773} & \multicolumn{1}{c}{29.82 / 0.8750} \\ \hline
% {\cmark}        & {\xmark}       & {\cmark}            & \multicolumn{1}{c}{29.94 / 0.8764} & \multicolumn{1}{c}{29.73 / 0.8741} \\ \hline
% {\xmark}        & {\cmark}       & {\cmark}           & 30.03 / 0.8774                      & 29.81 / 0.8756                      \\ \hline \hline
% {\cmark}        & {\xmark}       & {\xmark}           & 30.12 / 0.8783                      & 30.02 / 0.8784                      \\ \hline
% {\xmark}        & {\cmark}       & {\xmark}            & 30.16 / 0.8792                      & 30.11 / 0.8801                      \\ \hline
% {\cmark}       & {\cmark}       & {\xmark}           & 30.20 / 0.8799                      & 30.14 / 0.8808                      \\ \hline
% \end{tabular}%
% }
% \end{table}

\begin{table}[]
\centering
\setlength{\tabcolsep}{9pt}
\caption{The impact of different position embeddings and the pre-trained optical flow network. We compare various configurations on GoPro and Adobe datasets, following the setting of \textit{Average} in \Tref{tab:table1}. \textbf{O{$\cdot$}F} denotes the pre-trained optical flow network \cite{teed2020raft}, \textbf{B} represents {\bspline} and \textbf{F} represents {\fourier}. The first row shows the basic MoTIF configuration  \cite{chen2023motif}. Results are evaluated using PSNR (dB) and SSIM metrics.}
\label{tab:optical_abl}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc||cc}
\hline
\textbf{O{$\cdot$}F} & \textbf{B} & \textbf{F} & GoPro  & Adobe  \\ 
\hline 
\hline
{\cmark}   &  & & 30.04 / 0.8773 & 29.82 / 0.8750 \\ 
\hline
{\cmark} &  & {\cmark}  & 29.94 / 0.8764 & 29.73 / 0.8741 \\ 
\hline
{\cmark}  & {\cmark}  &   & 30.03 / 0.8774 & 29.81 / 0.8756 \\ 
\hline 
\hline
  &  &  {\cmark} & 30.12 / 0.8783 & 30.02 / 0.8784 \\ 
\hline
  & {\cmark} &  & 30.16 / 0.8792 & 30.11 / 0.8801 \\ 
\hline
 & {\cmark} & {\cmark} & \textbf{30.20 / 0.8799} & \textbf{30.14 / 0.8808} \\ 
\hline
\end{tabular}%
}
\end{table}

% \begin{table}[]
% \centering
% \caption{Comparisons of various configuration on GoPro and Adobe datset following the setting of -\textit{Average}. O{$\cdot$}F is pre-trained optical flow network \cite{teed2020raft}, B is {\bspline} and F is {\fourier}.}
% \label{tab:optical_abl}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|ccc||cc}
% \hline
% Methods & O{$\cdot$}F & B & F & Gopro  & Adobe  \\ 
% \hline 
% \hline
% Baseline \cite{chen2023motif} & {\cmark}   &  & & 30.04 / 0.8773 & 29.82 / 0.8750 \\ 
% \hline
% Baseline \cite{chen2023motif}-F & {\cmark} &  & {\cmark}  & 29.94 / 0.8764 & 29.73 / 0.8741 \\ 
% \hline
% Baseline \cite{chen2023motif}-B & {\cmark}  & {\cmark}  &   & 30.03 / 0.8774 & 29.81 / 0.8756 \\ 
% \hline 
% \hline
% Ours-F &  &  &  {\cmark} & 30.12 / 0.8783 & 30.02 / 0.8784 \\ 
% \hline
% Ours-B &  & {\cmark} &  & 30.16 / 0.8792 & 30.11 / 0.8801 \\ 
% \hline
% Ours &  & {\cmark} & {\cmark} & \textbf{30.20 / 0.8799} & \textbf{30.14 / 0.8808} \\ 
% \hline
% \end{tabular}%
% }
% \end{table}

%-------------------------------------------------------------------------



Additionally, we compare our model with C-STVSR methods in \Tref{tab:table2}, focusing on arbitrary-scales that were not seen during training. We perform experiments on GoPro dataset. Note that while TMNet supports continuous frame interpolation, it is limited to $\times\text{4}$ spatial super-resolution. Our results show that BF-STVSR achieves the best performance across all test cases, except for a minor disparity (0.03 dB lower PSNR) at $\times$6 temporal scale and $\times$6 spatial scale. This finding suggests that our {\bspline} effectively handles temporal interpolation even at distant time intervals.
Based on \Tref{tab:table2}, we present the performance degradation in PSNR and SSIM as the temporal scale increases from $\times $6 to $\times $12 and $\times $16 across various spatial scales in \Tref{tab:table-delta}. Our results demonstrate that MoTIF experiences a more pronounced performance drop than our model under challenging conditions. Specifically, at $\times $12 spatial scale, as the temporal scale increases from $\times $6 to $\times $12, MoTIF shows a degradation of approximately -4.02 dB, while our model degrades by around -3.63 dB, indicating an improvement of nearly 0.4 dB. This suggests that our method remains robust even under extreme conditions, with temporal intervals extending up to $\times $16.

%-------------------------------------------------------------------------

% \begin{table*}[]
% \centering
% \caption{ Ablation experiment on individual Mappers. Ours is original BF-STVSR, Ours-B only uses {\bspline} to map the motion vectors, reliability maps and Ours-F only use {\fourier} to map low resolution spatial features to high-resolution spatial features. Performance is evaluated using PSNR and SSIM metrics.}
% \label{tab:ablation1}
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{c|ccccc}
% \hline
%          & Vid4          & Gopro-\textit{Center} & Gopro-\textit{Average} & Adobe-\textit{Center} & Adobe-\textit{Average} \\
% \hline
% Ours & 25.80 / 0.7754 & \textbf{31.14} / \textbf{0.8893} & \textbf{30.20} / \textbf{0.8799} & \textbf{30.84} / \textbf{0.8877} & \textbf{30.14} / \textbf{0.8808}   \\
% Ours-B   & 25.79 / 0.7746 & 31.02 / 0.8875 & 30.12 / 0.8783 & 30.74 / 0.8852 & 30.02 / 0.8784   \\
% Ours-F   & \textbf{25.84} / \textbf{0.7764} & 31.11 / 0.8889 & 30.16 / 0.8792 & 30.82 / 0.8873 & 30.11 / 0.8801   \\
% \hline
% \end{tabular}%
% }
% \end{table*}


%-------------------------------------------------------------------------


%-------------------------------------------------------------------------
\begin{table*}[]
\centering
\caption{ Ablation study on the cross basis function configurations. Results are evaluated using PSNR (dB) and SSIM metrics. ``Ours-cross'' uses {\fourier} as temporal basis function and {\bspline} as spatial basis function. ``Ours-FF'' uses {\fourier} for both axes and ``Ours-BB'' uses {\bspline} for both axes. \textbf{Bold} indicates the best performance.}
\label{tab:ablation2_}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\hline
         & Vid4          & Gopro-\textit{Center} & Gopro-\textit{Average} & Adobe-\textit{Center} & Adobe-\textit{Average} \\
\hline
Ours        & 25.80 / \textbf{0.7754} & \textbf{31.14} / 0.8893 & \textbf{30.20} / \textbf{0.8799} & \textbf{30.84} / 0.8877 & \textbf{30.14} / 0.8808   \\
Ours-cross  & 25.78 / 0.7747 & 31.10 / 0.8892 & 30.17 / 0.8796 & 30.80 / 0.8876 & 30.10 / 0.8804   \\
Ours-FF     & 25.79 / 0.7750 & 31.12 / \textbf{0.8894} & 30.18 / 0.8798 & \textbf{30.84} / \textbf{0.8879} & 30.13 / \textbf{0.8809}   \\
Ours-BB     & \textbf{25.82} / 0.7753 & 31.07 / 0.8885 & 30.16 / 0.8793 & 30.77 / 0.8865 & 30.09 / 0.8797   \\
\hline
\end{tabular}%
}
\end{table*}

% \begin{table}[]
% \centering
% \caption{ Ablation study of the cross basis function. \textbf{Ours-cross} use {\fourier} as temporal basis function and {\bspline} as spatial basis function. Performance is evaluated using PSNR and SSIM metrics. The PSNR/SSIM values are slightly lower in \textbf{Ours-cross}, but the differences are minimal.}
% \label{tab:ablation2_}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|ccccc}
% \hline
%          & Ours          & Ours-cross & Ours-FF & Ours-BB  \\
% \hline
% Vid4        & 25.80 / \textbf{0.7754} & \textbf{31.14} / 0.8893 & \textbf{30.20} / \textbf{0.8799} & \textbf{30.84} / 0.8877    \\
% Gopro-\textit{Center}  & 25.78 / 0.7747 & 31.10 / 0.8892 & 30.17 / 0.8796 & 30.80 / 0.8876   \\
% Gopro-\textit{Average}     & 25.79 / 0.7750 & 31.12 / \textbf{0.8894} & 30.18 / 0.8798 & \textbf{30.84} / \textbf{0.8879}   \\
% Adobe-\textit{Center}     & \textbf{25.82} / 0.7753 & 31.07 / 0.8885 & 30.16 / 0.8793 & 30.77 / 0.8865   \\
% Adobe-\textit{Average}     & \textbf{25.82} / 0.7753 & 31.07 / 0.8885 & 30.16 / 0.8793 & 30.77 / 0.8865   \\
% \hline
% \end{tabular}%
% }
% \end{table}


% \begin{table}[h]
% \centering
% \caption{Ablation study of the cross basis function. \textbf{Ours-cross} use {\fourier} as temporal basis function and {\bspline} as spatial basis function. The PSNR/SSIM values are slightly lower in \textbf{Ours-cross}, but the differences are minimal.}
% \label{table:ablation2}
% \begin{tabular}{c|c|c}
% \hline
%               & \textbf{Ours} & \textbf{Ours-cross} \\ \hline
% GoPro-\textit{Center}     & 31.14 / 0.8893  & 31.10 / 0.8892 \\
% GoPro-\textit{Average}    & 30.20 / 0.8799  & 30.17 / 0.8796 \\
% Adobe-\textit{Center}     & 30.84 / 0.8877  & 30.80 / 0.8876 \\
% Adobe-\textit{Average}    & 30.14 / 0.8808  & 30.10 / 0.8804 \\ \hline
% \end{tabular}
% \end{table}


%-------------------------------------------------------------------------

\subsection{Qualitative results}
In \Fref{figure3}, qualitative results are shown, comparing our model with VideoINR and MoTIF. The results include interpolated frames for an in-distribution temporal scale ($\times$8), used during training (left), and an out-of-distribution temporal scale ($\times$6), unseen during training (right). For the in-distribution scale, BF-STVSR captures high-frequency details more effectively, particularly in the horse’s hooves and the striped shape of the handrails. For the out-of-distribution scale, BF-STVSR demonstrates superior performance in dynamic motion scenes, accurately interpolating edges of the text and the man’s face, where other methods produce blurry or ghosted frames. These results highlight our model’s ability to perform natural motion interpolation for moving objects while effectively preserving high-frequency details. 
Additionally, \Fref{fig:fig4} shows interpolated results at an extreme scale with a spatial scale of $\times$4 and a temporal scale of $\times$12. We include interpolated frames at sampled time points ($t = 0.25, 0.5, 0.75$) along with residual intensity maps compared to ground truth frames. Our method produces sharper and more accurate results than MoTIF, especially in areas like the tire and the region next to the car window. Additional results for all time coordinates are provided in the supplementary document. 
%-------------------------------------------------------------------------
% \begin{table}[]
% \caption{Performance comparison on the C-STVSR baselines for out-of-distribution scale (on Gopro dataset) with different basis function mapper. }
% \label{tab:table_abl_arbi}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cc|cccc}
% \hline
% \begin{tabular}[c]{@{}c@{}}Temporal Scale\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spatial Scale\end{tabular} &  Ours  &   Ours-cross  &   Ours-FF  & Ours-BB \\ 
% \hline
% \hline
% $\times 6$ & $\times 4$ & \textbf{31.68 / 0.9082} & 31.65 / 0.9077 & 31.66 / 0.9079 & - \\
% $\times 6$ & $\times 6$ & \textbf{29.44 / 0.8516} & 29.41 / 0.8515 & 29.43 / 0.8516 & - \\
% $\times 6$ & $\times 12$ & 25.78 / 0.7284 & 25.82 / 0.7320 & 25.77 / 0.7286 & - \\
% \hline
% $\times 12$ & $\times 4$ & \textbf{28.06 / 0.8287} & 28.03 / 0.8285 & 28.05 / 0.8288 & - \\
% $\times 12$ & $\times 6$ & \textbf{27.06 / 0.7961} &  27.05 / 0.7962 & 27.05 / 0.7962 & - \\
% $\times 12$ & $\times 12$ & \textbf{24.87} / 0.7096 &  24.89 / 0.7131 & 24.86 / 0.7099 & - \\
% \hline
% $\times 16$ & $\times 4$ & \textbf{26.40 / 0.7844} & 26.38 / 0.7844 & 26.39 / 0.7848 & - \\
% $\times 16$ & $\times 6$ & \textbf{25.81 / 0.7621} & 25.80 / 0.7623 & 25.77 / 0.7286 & - \\
% $\times 16$ & $\times 12$ & \textbf{24.22 / 0.6950} & 24.23 / 0.6984 & 24.21 / 0.6953 & - \\
% % \hline
% % \hline
% % $\times 6$ & $\times 1$ & - & - & - & 32.34 / 0.9545 & 34.77 / 0.9696 & - \\
% % $\times 1$ & $\times 4$ & - & - & 33.02 / 0.9206 & 32.26 / 0.9198 & 33.84 / 0.9328 & - \\

% \hline
% \end{tabular}%
% }
% \end{table}
%-------------------------------------------------------------------------


\subsection{Ablation Study} 


\paragraph{Optical Flow and Position Embeddings} \Tref{tab:optical_abl} compares model performance with and without pre-trained optical flow network, RAFT \cite{teed2020raft}, across different combinations of our proposed {\bspline} and {\fourier} modules. The first row shows the basic MoTIF \cite{chen2023motif} configuration. As seen in the second and third row, including the optical flow network with the proposed modules degrades performance. In contrast, directly using the proposed modules to extract spatial and temporal features, without the optical flow network, improves performance across all cases (last three rows). We attribute this improvement to the proposed modules facilitating the model's effective extraction and utilization of the rich information embedded within the video, enhancing its capacity to capture complex spatial and temporal features. 
In addition, the fourth and fifth row in \Tref{tab:optical_abl} represent the impact of the {\bspline} and {\fourier}, respectively. The fourth row is the result of using only {\fourier} for spatial feature encoding at BF-STVSR (last row) simply mapping the counterpart axis by concatenating latent features with target coordinates. which termed as Ours-F. The fifth row is the result of using only {\bspline} for temporal feature encoding at BF-STVSR (last row), which termed as Ours-B. As shown in the table, performance decreases when each mapper is used independently, but the best results are achieved when both mappers are integrated.

% \paragraph{Optical flow with proposed Mappers}  \Tref{tab:optical_abl} demonstrates the impact of incorporating the pre-trained optical flow network RAFT \cite{teed2020raft} as motion features, with or without the proposed mappers. The first row represents the baseline MoTIF configuration, where optical flows $M_{0\rightarrow1}, M_{1\rightarrow0}$ between reference frames, predicted by RAFT, are used to estimate intermediate motion vectors ($M_{0 \rightarrow t}^H, M_{1 \rightarrow t}^H$) without any positional encoding. In the first to third rows, it present the results based on MoTIF, combined with different mappers as indicated. In the fourth to last rows, following the BF-STVSR setup, intermediate motion vectors are predicted from the encoder output features using the specified mappers, with the last row representing the baseline BF-STVSR configuration. As shown, using RAFT's output with our proposed mappers leads to a performance degradation. In contrast, excluding RAFT's output improves performance, achieving the best results in the final configuration which is BF-STVSR setup (last row). This indicates that using ground-truth optical flow from a pre-trained network contrains the model's capability to learn the internal information of the video. 

% \paragraph{{\bspline} and {\fourier}}
% \Tref{tab:optical_abl} presents the results of an ablation study assessing the impact of each mapper. Ours-B and Ours-F correspond to configurations that use only the {\bspline} or {\fourier} for encoding temporal or spatial features, respectively, while simply mapping the counterpart axis by concatenating latent features with target coordinates. As shown in the table, performance decreases when each mapper is used independently, but the best results are achieved when both mappers are integrated.

% Ours-B utilizes only the {\bspline}, where spatial features are directly mapped to high-resolution features without any embedding process. Similarly, Ours-F employs only the {\fourier} in spatial axis, without any additional motion embedding, directly maps the queried coordinates with latent features to motion vectors and reliability maps. As shown in the table, the performance slightly decreases when each mapper is used separately, while it shows best performance when both mappers are integrated. %Thankfully, because of the strong embedding capacity of each mapper, the performance gap is very minimal. 
%-------------------------------------------------------------------------

% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%     \includegraphics[width=\linewidth]{fig/abl1_cropped2.pdf}

%    \caption{Qualitative results of large out-of-distribution scale that is $\times\text{4}$ for spatial and $\times\text{12}$ for temporal scale. We only represent the 3 intermediate times ($t= \text{0.25, 0.5, 0.75}$) and able to observe that our model generates the most accurate and clear intermediate frames compared to previous models.}
%    \label{fig:abl_fig}
% \end{figure}

%-------------------------------------------------------------------------

\paragraph{Different basis functions}
% We conduct ablation experiments by interchanging the basis functions of each axis and also by using the same basis function for both axes. In the variant Ours-cross, we utilize B-spline functions for spatial axis and Fourier functions for the temporal axis. In contrast, Ours-FF uses Fourier functions for both axes, while Ours-BB uses B-spline functions for both axes. For spatial {\bspline}, we estimate the coefficients and knots of B-spline basis function to represent spatial features. For temporal {\fourier}, we estimate the dominant frequency and amplitude of each reference frame to map each features to intermediate motion vectors and a reliability map. Additionally, we use a phase estimator, which takes the the video interval as input, similar to how the dilation estimator is used in {\bspline}. \Tref{tab:ablation2_} shows the quantitative results. Our proposed configuration, which uses B-spline for temporal representation and Fourier for spatial representation, achieves the highest performance. While the performance difference across these configurations is minimal (approximately 0.04dB), this suggests that  B-spline functions are particularly well-suited for modeling smooth, continuous temporal motion, while Fourier functions exel in capturing high-frequency spatial details. This alignment between basis functions and the intrinsic characteristics of each axis shows the effectiveness of our approach. 


We conduct additional experiments by varying the basis functions used for both axes (\Tref{tab:ablation2_}). In all configurations, the basis function model the spatial and temporal axes, while other components (\textit{e.g.}, linear projection for intermediate motion vectors and reliability maps) remain the same. Although the performance differences among these configurations are minimal (around 0.04 dB), we adopt the configuration using B-spline for temporal representation and Fourier for spatial representation, as it achieves the highest performance. % this suggests that  B-spline functions are particularly well-suited for modeling smooth, continuous temporal motion, while Fourier functions exel in capturing high-frequency spatial details. This alignment between basis functions and the intrinsic characteristics of each axis shows the effectiveness of our approach. 
%-------------------------------------------------------------------------

\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{fig/figure_limit_re_cropped.pdf}
   \caption{Qualitative comparison on a large motion case with a spatial scale of $\times 1$ and a temporal scale of $\times 8$. Three interpolation results at $t= \text{0.25, 0.5, 0.625}$ are shown.}
   \label{fig:limitations}
\end{figure}

%-------------------------------------------------------------------------



% Furthermore, Figure \ref{fig:abl_fig} shows the qualitative results betweent the Ours and Ours-cross. We can see that Ours interpolate the intermediate frames more smoothly, especially in dynamic motion. Specifically, the face of the man are distorted and the foot part are more blurry in Ours-cross.

\paragraph{Limitations} While our method demonstrates performance improvements, there still remain certain limitations. As shown in \Fref{fig:limitations}, existing C-STVSR models, including ours,  still struggle with handling large motion. %This limitation arises due to the small patch size of C-STVSR, which results in an inadequate receptive field. 
Moreover, the training process of C-STVSR models is time-consuming and computationally expensive. Addressing these challenges remains an open problem for future research.

% \section{Conclusions}
% We present a novel perspective to overcome the limitation of previous C-STVSR that naively use the INR for continuous representation without additional positional encoding. leveraging the power of positional encoding in C-STVSR by considering the spatial and temporal axes respectively regards to each characteristics. We ensure that when processing the spatial super-resolution, model have to be able to focus on high-frequency information. Also, when performing the temporal super-resolution, model should consider the motion of objects to move smoothly and non-uniformly rather than jerky or linearly. Therefore, instead of naively maps the neural representation using MLPs, we propose new pipeline named BF-STVSR, which consist of {\fourier} and {\bspline}. By using the {\fourier} as spatial basis function, we can capture high-frequency information from low-resolution images more effectively. Additionally, {\bspline} interpolates the motion features between the input frames smoothly by inherent feature of b-spline functions. We demonstrate the effectiveness of BF-STVSR by experiments and achieves the state-of-the-art performance on C-STVSR.

\section{Conclusions}
% In this paper, we introduce novel positional encoding modules, {\bspline} and {\fourier}, which use separate basis function for spatial and temporal axes. It is designed to reflect the characteristics of video data and overcome the limitations of previous C-STVSR methods. {\bspline} utilizes B-spline basis functions to interpolate temporal representations, providing a smooth and effective way to model motion features. Meanwhile, {\fourier} captures spatial features by estimating the dominant frequency information of the input video frames, which helps capture fine spatial details. Equipped with these proposed modules, our method, BF-STVSR, achieves state-of-the-art performance in C-STVSR, demonstrating the effectiveness of our approach.

In this paper, we proposed BF-STVSR, a novel framework for Continuous Spatial-Temporal Video Super Resolution (C-STVSR). We introduced two specialized position encoding modules: {\bspline}, which leverages B-spline basis functions for smooth and accurate temporal interpolation, and {\fourier}, which captures dominant spatial frequencies to effectively model fine-grained spatial details. Our analysis highlights that naive position encoding can degrade performance, particularly when paired with optical flow networks, emphasizing the importance of tailored encodings for spatial and temporal axes. Through extensive experiments, we show that BF-STVSR achieves state-of-the-art performance in PSNR and SSIM metrics across diverse datasets, demonstrating enhanced spatial detail, natural temporal consistency, and robustness under challenging conditions, including extreme out-of-distribution scales. 



% \paragraph{Acknowledgement}


